Learning Power Control Protocol for In-Factory 6G Subnetworks

In-X Subnetworks are envisioned to meet the stringent demands of short-range communication in diverse 6G use cases. In the context of In-Factory scenarios, effective power control is critical to mitigating the impact of interference resulting from potentially high subnetwork density. Existing approaches to power control in this domain have predominantly emphasized the data plane, often overlooking the impact of signaling overhead. Furthermore, prior work has typically adopted a network-centric perspective, relying on the assumption of complete and up-to-date channel state information (CSI) being readily available at the central controller. This paper introduces a novel multi-agent reinforcement learning (MARL) framework designed to enable access points to autonomously learn both signaling and power control protocols in an In-Factory Subnetwork environment. By formulating the problem as a partially observable Markov decision process (POMDP) and leveraging multi-agent proximal policy optimization (MAPPO), the proposed approach achieves significant advantages. The simulation results demonstrate that the learning-based method reduces signaling overhead by a factor of 8 while maintaining a buffer flush rate that lags the ideal "Genie" approach by only 5%.

==> dump.tex <==
%\subsection{Case A: Hierarchical Topology}  Figure \ref{f1} shows the system model for the hierarchical topology setup. In this setup, there is a gNB at the top which coordinates the APs which in turn coordinate the sensor-actuator units. Depending on use cases, subnetworks could have different QoS requirements. For example,  condition monitory, process automation and motion control applications could have latency requirements of 100ms, 50-3000ms and 10ms respectively \cite{8638027}. Where there are more than one sensor- actuator pairs in a subnetwork some kind of transmission scheduling is needed. To this end,  the aim is to maximize the probability of end to end transmission of each subnetwork meeting the control loop delay deadline. Doing so requires that the controller in the AP intelligently schedules transmissions within its network. Additionally meeting this aim will also need maximizing the APs access to the available shared channel. Both transmission scheduling and acces to the schared channel are responses to the signalling message exchange between APs and the gNB. It is assumed that the controllers/APs are half duplex devices.  If the uplink transmission rate of the $j_{th}$ sensor is given by $R_{j}$ and the downlink transmission rate of the AP in the downlink is $R_{AP}$ , then total delay of the control loop operation involving the $v_{th}$ packet from the $j_{th}$ is given by:

%\begin{equation}
%    t_{j}^{v} = \dfrac{A_{v}}{R_{j}} +  \dfrac{A_{v}}{R_{AP}} + \tau_{queue}^{j} + \tau_{queue}^{AP}
%\end{equation}


%where $A_{v}$  is the the packet size, $\tau_{queue}^{j}$ is the time between packet arrival at sensor j to packet transmission, $\tau_{queue}^{AP}$  is the time between packet arrival at the AP and the transmission of an AP generated control command carrying packet to an actuator. Each sensor-actuator pair is also also characterised by a  control loop  delay deadline, $\tau_{c}$. Hence again the aim is to maximize probability of end to end transmission of each subnetwork meeting the control loop delay deadline.

\subsubsection{Signalling messages}
There are uplink and downlink signalling messages that the APS will need to learn to use and interpret. The downlink message from the base station is:
\begin{itemize}
    \item Scheduling grant (SG)
\end{itemize}

whereas the uplink message from the AP are :
\begin{itemize}
    \item Scheduling request (SR)
\end{itemize}
The gNB exchanges allocation messages with the APs. The meaning of these messages are not known by the APs  and so the  APs need to learn how to interpret and so react to these messages from the gNB.  The communication action space of the $k_{th}$ AP is $u_{t}^{k} \in \{0,1\}$ for null message and SR.
For the gNB, the downlink message to the $k_{th}$ AP is given by $d_{t}^{k} \in \{0,1,2,...,M\}$  where $0$ means null message and the values between 1 and M are channel indices and indicate the service grant for the particular channel. 

The observation space can include the queue state at the sensor and the state of AP selected channel. $o_{t}^{k} = \{|D|,C\}$,  where  $|D|$ is the packets in the queue of the device and $C$ is the channel sate of the channel selected by the AP.

The gNB observes the channel with observation $ o_{t}^{AP} = \{c_{1}, c_{2},...,c_{M}, \mathcal{N}_{o}$ \}where $c_{i} \in \{o,k,N+1\}$ meaning idle channel, tansmission on $i_{th}$ channel by the $k_{th}$ device and transmission by more than one device on the ith channel respectively. $\mathcal{N}_{o}$ is the number of APs that transmit the command control packet within the delay budget.



%\subsection{Case B: Distributed Topology}
%For this case, we consider $M$ subnetworks each having an access point and $1/N$ device(s) that are coordinated by the access point as Figure \ref{f2} shows. The bandwidth available to the APs are divided into $F$ equal sized channels indexed as $f\in \mathcal{F} = \{1,2,...F\}$ each having a bandwidth of $W$ MHz. To access the channels, the APs exchange signalling messages to indicate the occupancy of the available channels. For example if AP, $k$ selects to use channel $f = 1$, it broadcasts a bit indicating the channel index. Other APs can chose to respond with the indices of  their occupied channels. The meaning of these messages are unknown to the APs and so their meaning need to be learnt by the APs. An AP's response to signalling messages from other APs are based on its experience as it explore their shared environment.  We assume that the APs communicate over a control channels, whereas APs and their associated sensors communicate over data channels. The AP to AP communication can be done via a side link. All the sidelink control channels are assumed to be perfect and so error free. 

%AP to AP Signalling messages are derived from a vocabulary set of size $2^L$ where $L$ is the maximum length of each signalling message. Hence the first goal is to evolve a signalling policy between APs to coordinate their  access to the shared data channel. The sidelink messages that APs send  are:

%\begin{itemize}
%    \item Channel occupancy request  (CoR)
%     \item Channel occupancy status (CoS)
%\end{itemize}
%Each AP also receives signaling messages from the sensors within its coverage: 
%\begin{itemize}
 %   \item Queue status (QS)
%\end{itemize}
On the other hand , for the $f_{th}$ data channel between the $m_{th}$ AP and the $n_{th}$ sensor associated with the $n_{th}$ subnetwork, 
 the signal to noise plus interference ratio (SINR) is given by :

\begin{equation}
     \gamma_{m,n,m}^{f} = \dfrac{g_{m,n,m}^{f}}{\sum_{m^{'}\in \mathcal{Y}_{mm^{'}}} g_{m,n,m^{'}}^{f}+ \sigma^{2}}
\end{equation}
, where $g_{m,n,m}^{f}$ is the received power on the link between the $m_{th}$ AP and the $n_{th}$ sensor in the $m_{th}$ sunetwork and is composed of sensor transmit power, large scale path loss, small scale fading and shadowing as in \cite{10118710}. $\sum_{m^{'}\in \mathcal{Y}_{mm^{'}}} g_{m,n,m^{'}}^{f}$ is the sum of all interfering signals from all transmissions in all $m^{'}\in \mathcal{Y}_{mm^{'}}$ subnetworks where $\mathcal{Y}_{mm^{'}}$ is the set of all subnetworks transmitting on the same $f$ channel as the $m_{th}$ subnetwork. Therefore the data rate of the $n_{th}$ sensor is given as:
\begin{equation}
    C_{m,n,m} \approx W\log(1 + \gamma_{m,n,m}^{f})
\end{equation}


\begin{figure} [!h]
    \centering
    \includegraphics[width=0.95\linewidth]{subnet_case_2.png}
    \caption{A network of M subnetwork  access points (AP) and N sensor/controller units. Signalling link are indicated by green arrows, measurements are indicated by the the blue arrow, control signals are indicated by the red arrows}
    \label{f2}
\end{figure}
 \subsubsection{Traffic Model}
 Within each subnetwork, uplink traffic is generated at the sensors using a Poisson process such that for the $n_{th}$ sensor in the $m_{th}$ subnetwork, the arrival rate  of each $e$ packet  is $\lambda = p_{e} \times T$,  where $p_{e}$ is the packet arrival probability of the $e_{th}$ packet and $T$ is the packet communication time. 
\subsubsection{Observation space }
In each time step, t, the environment delivers observations to each AP such that the observation 
 $o_{t}^{m} \in \mathcal{O^{AP}}= \{\mathcal{N}_{p},X\}$,  where $\mathcal{N}_{p}$ is the number of packets in the AP queue or could it be number of packets received within the deadline?,  $X$ is the channel sate of the channel selected by the $m_{th}$ AP. Values of $X$ include $X \in \{0,1\}$ which  mean idle channel, busy channel/collision in channel.
\subsubsection{Environmental action space}
These are the actions taken by the agents that have an impact on the environment. Each time step, each AP agent takes channel selection decisions for uplink communication within its subnetwork. Such action is given by $a_{t}^{m} \in \{ 1,2,..,F\}$ where the values $\{ 1,2,..,F\}$ is the index of the channel selected by the $m_{th}$ subnetwork.
\subsubsection{Communication action space}
Each AP take actions that do not have a direct impact on the environment but are rather signalling messages exxchanged between APs. 
$u_{t}^{k} \in (C_{r},C{s})$ where $C_{r} \in \{1,2,..F\}$ is the channel occupancy request for one for the channels and $C_{s} \in \{l_1,l_2,..l_M\}$ is the channel occupancy status for all the sensors where $l \in 1, 2,F...,$ 

 








%\section{Problem Formulation}
%For this paper, the goal is to ensure the continuous operation of the controlapplications supported by sensors in the subnetwork while minimizing signaling overhead to exchange information. We formulate this as problem of minimizing the probability of burst error exceeding the survival time of all sensors in all the subnetworks:
%To make RL agent (in this case the gNB and controllers) learn the scheduling policy, channel access policy and the signalling policy that optimize the continuous operation of the network  or the communication service availability and so minimize operation downtime. We can formulate this problem as a MARL where the gNB and the controllers are RL agents that learn to communicate about channel access.  It can also be fashioned as a MARL problem where the APs learn to communicate with each other to evolve a MAC protocol. In which case there is no central entity like a gNB rather each AP is equipped with an interface that that can utilize any of the available channels, however to limit inter subnetwork interference and so ensure continuous network operation. A key aim of scheduling is to get the packet through successfully and where each sensor has a survival time cap on its transmission, factoring in this parameter provides a kind of fairness to the setup. 

%throughput maximization problem scaled by the sum survival time of each time slot. Thus the problem is formulated as :

%\begin{equation}
%\begin{aligned}
%\min_{\pi_{S}, \pi_{A}, \pi_{H} } \Sigma_{k = 1}^{M} \Sigma_{i = 1}^{N} Pr(BL_{i,k} > \tau_{surv_{i,k}}) \\
%\label{E1}
%\end{aligned}
%\end{equation}

%\begin{equation}
%Min :\Sigma_{k = 1}^{M} \Sigma_{i = 1}^{N} Pr(BL_{i,k} > \tau_{surv_{i,k}}),
%\end{equation}
%where $BL_{i}$ is the burst error length for transmission of the $i_{th} $ sensor, $\pi_{S}$ is the signalling policy, $\pi_{A}$ is the channel access policy and $\pi_{H}$ is the scheduling policy which the access points or controllers will need to learn. The optimal policy being, $\pi^{*} =\{\pi_{S}^{*}, \pi_{A}^{*},\pi_{H}^{*}\} $.  Some terms are associated with this work are defined in the item list below:
%\begin{itemize}
%    \item \textbf{Burst error length ($BL_{i}$}) is the number of consecutive erroneous reception at the end of a communication cycle which is made of many communication time steps.
    %\item \textbf{Erroneous reception} occurs when (a) a device with packets to transmit in a given time step is not scheduled and so the packet is dropped (b) when a packet is transmitted but the rate is less than a set threshold.
%    \item \textbf{Time To Failure (TTF) - $<3GPP>$} is the duration between two or failure events. A failure event happens when the burst length is greater than the survival time. An average of various Times To Failure is called Mean Time Before Failure. 
     %\item \textbf{Time To Failure (TTF) - } for the purpose of this work is the time between the last last error event and communication service unavailability. Specifically this is the difference between the number of consecutive error events and the survival time. $TTF = \tau_{surv} - \mathrm{e}_{i}$. 
     %It is clear to see that where the $\tau_{surv}$ is 0, the TTF is negative.
    %\item \textbf{Communication Service Availability (CSA)} This is a measure of the times the communication service was delivered based on the target QoS. From the perspective of survival time, this is a measure of the times when the survival time condition was not violated. 
%\end{itemize}



%\section{Subnetwork Traffic }
%The traffic type considered is meant for control loop operations and real time traffic. Each sensor/actuator periodically generates packets and transmits same to the controller with a transfer interval or periodicity, $P_{i}$. Each of the sensors is also characterises by  survival time. The survival time may be same as or greater than the periodicity. 
%\begin{figure} [!h]
  %  \centering
 %   \includegraphics[width=0.85\linewidth]{traffic_image.png}
  %  \caption{Periodic Traffic for 4 sensors having periodicity of $P_{i} = 0,1,3,2$ }
  %  \label{f3}
%\end{figure}

%\subsection{Signalling Messages}

%\begin{table*}
%\caption{Subnetwork MAC Protocol Learning} %title of the table
%\centering % centering table
%\begin{tabular}{|l|l|l|} % creating eight columns
%\hline\hline %inserting double-line
%Architecture & Fig. \ref{f1}&Fig. \ref{f1a}\\
%\hline
%Signalling & UL- channel Request (CR) & Channel Free (CF), \\
%Messages& DL- channel Grant (CG) & Channel UnFree(CU)\\
%& \{$\mathcal{M}_{UL} = \{0,1\}^{L}_{1},\mathcal{M}_{DL} = \{0,1\}^{L}_{1}$& \{ $\mathcal{M}_{CL} = \{0, 1}$\}^L_{1} \\
%\hline
%Channel Access&AP learns this policy , \pi_{AP}&AP learns this policy , \pi_{AP}\\
%Policy 
%&following signalling or not&following signalling or not\\

%\hline
%Scheduling Policy&$\tau_{surv}$-aware&$\tau_{surv}$-aware\\
%\hline
%MARL Agent&APs and gNB &APs\\
%\hline
%RL Technique&Actor - Critic Network&Actors only network\\
%\hline
%Observation &  o_{gNB}(t)    = \begin{cases} 0 & idle, \\ 1 & busy\end{cases}&\\
%Space&&o_{AP}(t)    = \begin{cases} 0 & idle,\\ 1  & busy, \\ $[q_{N}(t)]$ & \forall d,\\ $[TTF_{N}(t)]$  & \forall d \\$[\gamma_{N}(t)]$  & \forall d 
% \end{cases}\\
%&o_{AP}(t)    = \begin{cases} $[q_{N}(t)]$ & \forall d,\\ $[TTF_{N}(t)]$  & \forall d ,\\$[\gamma_{N}(t)]$  & \forall d  \end{cases}&\\
%\hline
%Action &a_{AP} (t)   = \begin{cases} 0 & unschedule\\ 1  & schedule,\end{cases} &a_{AP}(t)    = \begin{cases} 0 & unschedule\\ 1  & schedule,\end{cases}\\
%Space&&\\
%\hline
%Reward&r_{AP}(t)   = \begin{cases} +1, & 1 \cap 2 \\0 & 1 \cup 2\\ -1  & otherwise,\end{cases}&r_{AP}(t)    = %\begin{cases} +1 & optimal^{*}\\ -1  & suboptimal, \end{cases}\\
%&1. \Sigma_{i}^{N} (TTF)< 1/N\Sigma_{i}^{N} (\tau_{surv_{i}}) &\\
%&2. $R > = R_{th}$&\\
%\hline
%State Space &s_{gNB}(t) = \{o_{gNB}(t),..., o_{gNB}(t-k),  m_{AP}^{UL}(t),..., &s_{AP}(t) = \{o_{gNB}(t),..., o_{gNB}(t-k), \\
%&m_{AP}^{UL}(t-k), m_{gNB}^{DL}(t),..., m_{gNB}^{DL}(t-k), \}&m_{AP}^{SL}(t),..., m_{AP}^{SL}(t-k)\\
%&&a_{AP}(t),..., a_{AP}(t-k)\}\\
%&s_{AP}(t) = \{o_{gNB}(t),..., o_{gNB}(t-k),  m_{AP}^{UL}(t),..., &\\
%&m_{AP}^{UL}(t-k), m_{gNB}^{DL}(t),..., m_{gNB}^{DL}(t-k), &\\
%&a_{AP}(t),..., a_{AP}(t-k)\}&\\
%\hline
%MARL&gNB and APs are RL agents learning a MAC protocol&APs are RL agents learning a MAC protocol\\
%&APs learn when to schedule&APs learn when to schedule\\
%&and how to schedule&how  to schedule\\

%\hline
%Approach&ACN&DQN\\
%\hline
%Objective Fxn&\begin{equation}
%Maximize :\Sigma_{k = 1}^{M} \Sigma_{i = 1}^{N} Pr(BL_{i,k} < \tau_{surv_{i,k}}),
%\end{equation}&\begin{equation}
%Maximize :\Sigma_{k = 1}^{M} \Sigma_{i = 1}^{N} Pr(BL_{i,k} < \tau_{surv_{i,k}}),
%\end{equation}\\
%\hline
%\end{tabular}
%\label{T1}
%\end{table*}
%\section{An Example}
%Consider a network with device $d_{i} , i= \{1, 2, . . N\}$ having a periodicity or transfer interval of $P_{i} = 1, 2,4,3$ as shown in Figure \ref{f3} and communication cycle of 10 time steps. Let the $\tau_{1}$ be 0 and $\tau_{2}$ be 3 time steps respectively. If in the second and eight time steps, the device 1 is either not scheduled or its packet is not received correctly, then the $CSA$ is 0.8 implying that out of ten time steps, the $\tau_{surv}$ condition was met 8 times. The TTF here is -2 for each of the error events because given an error event at time steps 2 and 8, with a $\tau_{surv}$ of 0, the TTF are both -2.

%Moreover the TTF is is 6 time steps and the $BL_{1}$ is 1. 

%Considering the forgoing there are counters that need to be implemented. 
%\begin{itemize}
%    \item Counter for the number of times a device with packets is not scheduled.
%    \item Counter for the number of times a scheduled packet is not received correctly.
%    \item Counter for the number of times error events (the first two) exceed the survival time. With this we find the objective function, $Pr(BL_{i} < \tau_{surv_{i}})$
%\end{itemize}
%\begin{equation}
%Maximize : \Sigma_{t = 1}^{T} \Sigma_{i=1}^{N} \dfrac{a(t)R_{i}(t)}%{\Sigma_{i=1}^{N} \tau_{i}(t)}
%\end{equation}
    
%\begin{gather}
%    \max \quad \Sigma_{t = 1}^{T} \Sigma_{i=1}^{N} \dfrac{a(t)R(t)}{\Sigma_{i=1}^{N} \tau_{i}(t)}                      \nonumber\\
%    \begin{aligned}
%    \end{aligned}
%\end{gather}


%\section{MARL }
%The formulated problem in equation \ref{E1} can be cast as a multi agent reinforcement learning where the gNB and APs in Case A; and the APs in case B. In case A, the gNB and APs need to cooperate to learn  a signalling policy between them. The APs also need to learn when to allow uplink transfer of packets from devices within its subnetwork and how to schedule these devices for packet transfer.
%The features characterising the MARL are described as follows:
%\subsection{Action Space}
%At a time step t, the $k_{th}$ AP selects an action $a_{t}^{k}$  which could assume values $\{0, 1\}$ meaning do nothing/don't schedule, schedule subnetwork transmission/receive transmissions from scheduled sensor-actuator pair. For ease of notation, let $a_{t}^{k}$ be expressed as $a^{k}$ such that $a^{k} = \{a_{1}^{k},a_{2}^{k},a_{2}^{k}, . . .,a_{n}^{k} \}$ is the sensor scheduling vector for the $k_{th}$ subnetwork. And so the joint action space combining the actions of all the APs is given by $\textbf{a}_{t} = \{a_{t}^{1}, ..., a_{t}^{M} \} \in \mathcal{A}$. 
%\subsection{Signalling  Messages} 
%Downlink and uplink signalling messages are sent by the gNB and the APs respectively. At each time step t, the $k_{th}$ AP sends an uplink signalling message to the gNB, $l_{t}^{k}$ with values $\{0, 1\}$ do nothing and channel grant respectively. The joint uplink messages for all the APs in the network is $\textbf{l}_{t} = \{l_{t}^{1}, ..., l_{t}^{M} \}$ . Similarly the $k_{th}$ AP also receives a downlink signalling message from the gNB given by $m_{t}^{k}$ with possible values of \{0,1\} corresponding to do nothing and channel grant respectively. Hence the joint downlink message set is given by, $\textbf{m}_{t} = \{m_{t}^{1}, ..., m_{t}^{M} \}$.
%\subsection{Local state space}
%This refers to the observation which each agent is presented with by the environment. Per time step t, the $k_{th}$ AP observes $o_{t}^{k}$ given by, $o_{t}^{k} = \{q_{t}^{k}, TTF_{t}^{k}, \gamma_{t}^{k}, m_{t}^{k} \}$
%\[o_{t}^{k}    = \begin{cases}  $q_{t}^{k}$ & \forall d\in N,\\ $TTF_{t}^{k}$  & %\forall d\in N\\$\gamma_{t}^{k}$  & \forall d\in N ,
% \end{cases}\]
%where $q_{t}^{k}$ is the packet transfer indicator received by the $k_{th}$ AP from all $N$ devices in its subnetwork, $TTF_{t}^{k}$ is a set of the time to failure received by the $k_{th}$ AP from all $N$ devices in its subnetwork and $\gamma_{t}^{k}$ is the set of signal to noise ratios from all $N$ devices in the $k_{th}$ subnetwork. $m_{t}^{k}$ is the downlink signalling message observed by the $k_{th}$ AP.
%Similarly the gNB receives observation per time step with values \{0, 1\} corresponding to idle channel and non-idle channel respectively. 
%\subsection{Global State space}
%The local state space is a subset of the environment's global state. At time step t, the global state, $s_{t} \in \mathcal{S}$ consists the joint action, $\textbf{a}_{t}$ and local observation, $o_{t}$ and signalling messages $\textbf{m}_{t}$ and $\textbf{l}_{t}$. i.e $s_{t} = \{\textbf{a}_{t}, o_{t}, \textbf{m}_{t}, \textbf{l}_{t}$\}
%\subsection{Reward Function}
%For each action taken $a_{t}^{k} $, all  agents receive the same reward, where the reward function is given by:


%\[r_{t} \in \mathcal{R}   = \begin{cases} +1, & \text{if   }  1 \cap 2 \\0 &  \text{if   } 1 \cup 2\\ -1  & otherwise,\end{cases}\]
%where,
%\begin{itemize}
%    \item 1. $\dfrac{1}{N} \Sigma_{i}^{n<N} (TTF_{i}) = min({TTF_{i}})_{1}^{N}$ and
 %   \item 2. $ \dfrac{1}{N} \Sigma_{i}^{n<N}R_{i} > = R_{th}$.
%\end{itemize}
%Condition 1 is a scheduling condition which ensures that the average time to failure of all scheduled sensors is less than the minimum survival time of the scheduled sensors. In meeting this condition, priority is given to packets with less TTF and so the likelihood of shutdown of machine operation is reduced. Condition 1 can be tasking especially at the first time slot where the $TTF$ is not yet known. So for this first time slot, the $t_{surv}$ is used.
%Condition 2 is a channel access condition. This condition ensures that the average rate of packet transmission is greater than a threshold rate ($R_{th}$)
%The first element in the reward set shows that each agent is rewarded with $+1$ when the agent meets both a channel access and scheduling criteria. When the agent meets either a scheduling or channel access criteria, it is rewarded with $-1$. When none of this happens, the agent receives $0$ as a reward.

%The action space, state space, observation space etc can be applied to Case B in Figure \ref{f1a} with some modifications. It is noteworthy that since $M$ subnetworks request for ($F< M$)  radio resources from the gNB per time step, the gNB needs a criteria for channel allocation. To keep the analysis tractable, we consider the case where gNB ranks the subnetworks based on SINR achieved in the last time step and selects the first F subnetworks. An example signalling diagram showing the flow of control messages and packet transmission are shown in Figure \ref{sig} for 3 time steps. The links between the APs and the gNB are control channels and control messages are exchanged on theses links. The links between each AP and its subnetwork are data links. 

%\begin{itemize}
%    \item The action set, $c_{i}(t) = \{ 0, 1 \}$ where 0 refers to transmit/schedule for transmission and 1 refers to stay idle/dont schedule. Hence the optimal policy is when for each time slot the the sensors are scheduled such that the probability that the burst error length is greater than the survival time is minimized. 
    %Transmit, Listen(stay idle) for scheduling grant/ACK, send transmit request or grant. For the $i_{th}$ UE, the action set $c_{i}(t) = \{0, 1\}$ for idle, transmit such that the action set for all UEs is $\textbf{c(t)} = {c_{1}(t), ..., c_{N}(t)  }$. If the control plane is included, control action space will have values of \{idle, RTS/SR \}

    %\item For the centralised implementation, - Unschedule, Schedule,  send ACK  \{0,1,2\}
    
%\end{itemize}
%In each time step, the environment presents the agent with observations which influence their actions. Depending on the considered assumptions, the observation space can be synonymous with the state space, or the state space can be a subset of the observation space. For the later case, the problem becomes a partially observable MDP and for the later case, simply an MDP.
%\begin{itemize}
    %\item For a decentralised Implementation where the sensors are the 
%    agents,- the state in each time step can be designed as having option: channel is busy $S(t) = 1$, channel is idle  $S(t) = 0$; $s_i(t) = [0, 1]$ such that the aggregated state space is $s_i(t) = \{s_1(t), s_2(t),..., s_N(t)\}$
%    \item  The state in each time step can be designed as containing: - packet transfer indicator $q_{i}(t) \in Q_{N} =\{0,1\}$, sensor-to-AP SINR $\gamma_{i}(t) \in \Gamma_{N} $, time to fail, $f_{i}(t) \in F_{N}(t) $. Hence the state space can be expressed as : $S =\{q_{1}(t),..,q_{N}(t) , \gamma_{1}(t),..., \gamma_{N}(t), f_{i}(t),...,f_{N}(t)   \}$.
    
    %The global state consist of the joint action space and the signalling or control messages. $s_i(t) = \{q_1(t),..., q_N(t), g_i(t),..,g_i(t), \gamma_{1}(t),.., \gamma_{N}(t), c_{1}(t), ..., c_{N}(t)  \}$. The local observation of each sensor is $\{ s_i(t) = q_i(t), \gamma_{i}(t),  g_i(t)\} $
%\end{itemize}


%\section{Action Space }
%\begin{itemize}
%    \item The action set, $c_{i}(t) = \{ 0, 1 \}$ where 0 refers to transmit/schedule for transmission and 1 refers to stay idle/dont schedule. Hence the optimal policy is when for each time slot the the sensors are scheduled such that the probability that the burst error length is greater than the survival time is minimized. 
    %Transmit, Listen(stay idle) for scheduling grant/ACK, send transmit request or grant. For the $i_{th}$ UE, the action set $c_{i}(t) = \{0, 1\}$ for idle, transmit such that the action set for all UEs is $\textbf{c(t)} = {c_{1}(t), ..., c_{N}(t)  }$. If the control plane is included, control action space will have values of \{idle, RTS/SR \}

    %\item For the centralised implementation, - Unschedule, Schedule,  send ACK  \{0,1,2\}
    
%\end{itemize}

%\section{Reward Function}
%For each action taken $c_{i}(t) $, if the action follows the optimal policy of optimizing the objective function, there is a reward, else there is a punishment. Thus
%\begin{equation}
 %%   r_{t}= \begin{cases} +1 , & if \, $c_{i}(t) == c_{i}^{*}(t)$ \\ 
  %  -1, &otherwise\\

   % \end{cases}
%\end{equation}


%Per time slot these parameters can be calculated
%\begin{itemize}
%    \item Rate ($R(t)$)
%    \item Scheduling vector ($a(t)$)
%    \item Total Survival time of scheduled nodes ($\Sigma_{i=1}^{N} \tau_{i}(t)$) - Reward should be higher when the total survival time of scheduled nodes is small
%\end{itemize}
%Possible Reward functions 
%\begin{itemize}
%    \item $a(t)R(t) - \Sigma_{i=1}^{N} \tau_{i}(t)$
%    \item $\dfrac{a(t)R(t)}{\Sigma_{i=1}^{N} \tau_{i}(t)}$
%\end{itemize}


%\begin{figure}
%    \centering
 %   \includegraphics[width=0.95\linewidth]{signalling_diagram.png}
  %  \caption{An Example Signalling Diagram for the Proposed System Model}
   % \label{sig}
%\end{figure}


%\section{Reinforcement Learning}
%For this work we consider a policy gradient based RL approach, specifically we model our problems as  a multi agent RL characterised by $(\mathcal{M}, \mathcal{A},\mathcal{S}, \mathcal{O},\pi_{i},\mathcal{R}(t+1))$ for which we propose a actor-critic network. Like the work in \cite{Mota2021TheEO}, a centralised training and distributed execution approach is adopted to learn the optimal policy . Each agent has a centralised critic network that calculates the Q-value for the action of the agent, and an actor network that provides the action for agent. 
%\subsection{Actor Critic Network}
%Reinforcement Learning can be approached from the value approximation approach or the policy gradient approach. The actor - critic network combines both approaches such that the actor network learns from the state space and outputs the probabilities of each action. The critic network on the other hand uses both observations from the environment and the output from the actor network to determine the future rewards of each action. Basically the actor is the policy function and the critic is the value function. Details of the Actor Critic network is shown in the diagram in Figure \ref{f2}. 


%\begin{itemize}
%    \item The current state $s(t)$ from the environment is fed as input into the  Critic while the local observation is fed  $o_{i}(t)$ into each Actor
%    \item The Actors outputs the probabilities of each possible action and the 'best' action ($c(t)$)
%    \item The Critic uses the state ($s(t)$) to calculate the Q-value $\mathcal{Q}(s(t), c(t))$
%    \item The environment outputs a new state $s(t+1)$, observations $o_{i}(t+1)$ and reward $\mathcal{R}$(t+1).
%    \item The actors update their parameters based on the Q-value, and outputs the new action probabilities given the new observation 
%    \item The critic updates its parameters based on the Q-value
%\end{itemize}

%\begin{figure} [!h]
%    \centering
%    \includegraphics[width=0.85\linewidth]{actor_critic.jpg}
%    \caption{MR Actor Critic Network}
%    \label{f2}
%\end{figure}
%\subsection{Proposed Implementation} This will be implemented in Python. The functions to build are:
%\begin{itemize}
    
%    \item A function to generate the locations and packets per time step
%    \item A function to generate the SINRs of the sensors to the AP
%    \item Actor network
%    \item Critic network
%    \item Reset Function returns the reward to zero at the end of an episode. Since the location of the sensors are random per time step, the sensor locations are not explicitly defined in the rest fxn
%    \item Environment - item 1, 2 and 5 are part of the environment.
%\end{itemize}
%\section{Performance Metrics}
%\begin{itemize}
%    \item Communication Service Availability
%\end{itemize}
% Loading bibliography database
%\bibliography{cas-refs}
